QuickLLaMA: Query-aware Inference Acceleration for Large Language Models

The capacity of Large Language Models (LLMs) to comprehend and reason over long contexts is pivotal for advancements in diverse fields. Yet, they still stuggle with capturing long-distance dependencies within sequences to deeply understand semantics. To address this issue, we introduce Query-aware Inference for LLMs (Q-LLM), a system designed to process extensive sequences akin to human cognition. By focusing on memory data relevant to a given query, Q-LLM can accurately capture pertinent information within a fixed window size and provide precise answers to queries. It doesn't require extra training and can be seamlessly integrated with any LLMs. Q-LLM using LLaMA3 (QuickLLaMA) can read Harry Potter within 30s and accurately answer the questions. On widely recognized benchmarks, Q-LLM improved by 7.17% compared to the current state-of-the-art on LLaMA3, and by 3.26% on Mistral on the $\infty$-bench. In the Needle-in-a-Haystack and BABILong task, Q-LLM improved upon the current SOTA by 7.0% and 6.1%. Our code can be found in https://github.com/dvlab-research/Q-LLM.

==> tables/token-level.tex <==
\begin{table*}[t]
    \centering
    \small
    \begin{tabular}{l|rrrr|rrrr}
    \toprule 
    Dataset    & Original & Yarn$^*$ &	PI & NTK  & Infinite & Stream &	InfLLM & \name \\ \midrule
    Context Window %& 128k 
                    & 32K & 128K & 128K & 128K & 6K & 6K & 4K + 2K & 4K + 2K  \\ 
    Attention Type %& --   
                    & Full & Full & Full & Full & Window & Window & Window & Window \\\midrule
    NarrativeQA   & 20.66 & 19.67 & 23.47 & 22.67 & 18.44 & 17.92 & 22.12 & 	\textbf{26.33}  \\

    Qasper        & 29.14 & 11.10 & 29.36 & 29.90 & 30.02 & 30.05 & 29.33 & \textbf{33.35} \\

    MultiFieldQA
                    & 47.39 & 35.06 & 46.47 & 46.41 & 39.05 & 39.09 & 47.42 & 	\textbf{49.25} \\

    HotpotQA      & 37.60 & 11.94 & 37.33 & 35.18 & 32.02 & 32.18 & 36.56 & \textbf{41.79} \\

    2WikiMQA      & 22.54 & 12.02 & 22.19 & 21.71 & 22.27 & 21.83 & 22.31 & 	\textbf{27.41} \\

    Musique       & 18.50 & 7.52  & 18.80 & 19.45 & 15.81 & 14.71 & 17.68 & \textbf{19.74} \\

    GovReport     & 31.03 & 29.46 & 32.36 & 32.86 & 29.74 & 29.83 & \textbf{31.03} & 28.96 \\ 

    QMSum         & 23.84 & 21.53 & 23.58 & 23.16 & 21.92 & 21.94 & 23.49 & \textbf{23.88} \\

    MultiNews     & 26.65 & 16.04 & 26.62 & 26.69 & 26.65 & 26.64 & \textbf{26.70} & 24.96 \\

    TREC          & 71.00 & 68.50 & 71.50 & 71.50 & \textbf{70.00} & 70.00 & 69.00 & \textbf{71.00} \\

    TriviaQA      & 86.22 & 88.21 & 88.86 & 89.31 & 85.22 & 85.57 & \textbf{86.67} & 86.06 \\

    SAMSum        & 42.11 & 26.52 & 42.58 & 41.55 & 41.60 & 41.31	& 42.52 & \textbf{42.88} \\
    PassageRetrieval
                    & 89.02 & 16.25 & 89.10 & 92.42 & 42.80 & 42.17	& 64.00 & \textbf{86.60} \\
	
    LCC           & 57.33 & 66.39 & 55.90 & 55.07 & \textbf{57.12} & 55.38 & 56.67 & 52.01 \\

    RepoBench-P   & 54.27 & 55.82 & 52.46 & 50.33 & \textbf{53.43} & 51.46 & 52.97 & 	48.16 \\ \midrule
    Average       & 43.82 & 32.40 & 44.04 & 43.88 & 39.07 & 38.67 & 41.90 & \textbf{44.16} \\
    \bottomrule
    \end{tabular}
    \caption{The results of \basemistral. The $95$\% quantile for Long-Bench is $31$K.  The context window size for InfLLM and \name is denoted as \textit{local window size + selected memory size}.}
%    \vspace{-1em}
    \label{tab:token-level}
\end{table*}
